Physics-based Shadow Image Decomposition for Shadow Removal

We propose a novel deep learning method for shadow removal. Inspired by physical models of shadow formation, we use a linear illumination transformation to model the shadow effects in the image that allows the shadow image to be expressed as a combination of the shadow-free image, the shadow parameters, and a matte layer. We use two deep networks, namely SP-Net and M-Net, to predict the shadow parameters and the shadow matte respectively. This system allows us to remove the shadow effects from images. We then employ an inpainting network, I-Net, to further refine the results. We train and test our framework on the most challenging shadow removal dataset (ISTD). Our method improves the state-of-the-art in terms of root mean square error (RMSE) for the shadow area by 20\%. Furthermore, this decomposition allows us to formulate a patch-based weakly-supervised shadow removal method. This model can be trained without any shadow-free images (that are cumbersome to acquire) and achieves competitive shadow removal results compared to state-of-the-art methods that are trained with fully paired shadow and shadow-free images. Last, we introduce SBU-Timelapse, a video shadow removal dataset for evaluating shadow removal methods.

==> sub.tex <==

\section{Shadow Matte Interpolation for Shadow Removal on Images with Arbitrary Sizes.}
\label{sec:sizes}

Our method can remove the shadows on images with arbitrary sizes by interpolating the shadow mattes. In this section, we compute the shadow parameters and shadow mattes from the input images of size $256\times256$. We then use the computed shadow parameters and shadow mattes to remove the shadows on the input images of size $480\times640$. In order to do so, we interpolate the computed shadow matte to this size using bi-linear interpolation. We keep the shadow parameters the same since the linear transformations that relight the shadow areas are unchanged when the images are resized.

Figure \ref{fig:highres} illustrates the effect of this method. The second column shows the outputs of our model at $256\times256$. We interpolate the computed shadow mattes to the size of $480\times640$ to output the images in the third column.  As can be seen, the shadow parameters and shadow matte computed from a resized input image ($256\times256$) can be used to effectively remove the shadows in the input images at the original scale.

We further compare the shadow removal performance of our methods to other state-of-the-art methods on the ground truth images at the original scale ($480\times640$) in Table \ref{tab:highres}. Note that in the main paper, all images are resized to $256\times256$.  Each method originally outputs the results at a different size, which shown in the second column. We resize all images to $480\times640$ using bi-linear interpolation. For our methods, we compute the shadow parameters and shadow matte using only the input images of size $256\times256$. We then interpolate the computed shadow mattes to the size of  $480\times640$ to output the shadow-free images at this size, denoted as ``SP+M-Net (S.Matte Interp.)'' and ``SP+M-Net Aug. (S.Matte Interp.)''. The results show that by interpolating the shadow mattes, our method can effectively remove the shadows on images at different scales. This could be useful when computational resources are limited.

\begin{table}[]
\centering
\caption{\textbf{Shadow removal results of our networks in comparison with state-of-the-art methods for shadow removal on the ground truth images at the original scale ($480\times640$).} The metric is RMS error (the lower, the better). The RMS errors are shown for the shadow area, non-shadow area, and the whole image. All images are resized to $480\times 640$ via bi-linear interpolation. For our methods, we compute the shadow parameters and shadow mattes using only the input images of size $256\times256$. We then interpolate the computed shadow mattes to the size of  $480\times640$ to output the shadow-free images at this size, denoted as ``SP+M-Net (S.Matte Interp.)'' and ``SP+M-Net Aug. (S.Matte Interp.)''.}
\begin{tabular}{lcccc}
\toprule
Methods              & Output size      & Shadow& Non-Shadow& All  \\ 
\midrule
Input Image          &     & 40.4  & 3.3 & 9.1\\ 
\midrule
Yang \etal~\cite{Yang12}   &$600\times600$              & 25.3  & 15.2 & 16.8\\ 
Guo \etal~\cite{guoPami}    &$640\times640$              & 22.3  & 4.3 & 7.1\\ 
Wang \etal \cite{Wang_2018_CVPR} &$256\times256$   & 14.0  & 8.6 & 9.5\\ 
Gong \etal~\cite{Gong16}   &$480\times640$         & 14.4  & \textbf{3.4} & 5.1\\ 
\midrule
%\multicolumn{4}{c}{Our method trained on the ISTD dataset \cite{Wang_2018_CVPR}}\\
SP+M-Net &$256\times256$  & 9.0  &4.6 &5.3\\ 
SP+M-Net (S.Matte Interp.) &$480\times640$    & 8.5  &3.6 &\textbf{4.4}\\
\midrule
SP+M-Net Aug. &$256\times256$  & 8.5  &4.7 &5.3\\ 
SP+M-Net Aug. (S.Matte Interp.) &$480\times640$    & \textbf{8.0}  &3.7 &\textbf{4.4}\\
\midrule
%SP+M-Net GT Mask. & 7.4  &2.8 &3.6\\ 
%SP+M-Net + GT Mask  & 7.0  &2.9 &3.5\\\hline
\end{tabular}
\label{tab:highres}
\end{table}



\def\subFigSzab{\textwidth}
\def\subboxsize{0.23\subFigSzab}
\begin{figure}[]
 \centering
    \includegraphics[width=0.9\textwidth]{fig/highres/112-2.png}
    \includegraphics[width=0.9\textwidth]{fig/highres/114-4.png}
    \includegraphics[width=0.9\textwidth]{fig/highres/120-10.png}
    \includegraphics[width=0.9\textwidth]{fig/highres/122-4.png}

    \makebox[\subboxsize]{Input Image}
    \makebox[\subboxsize]{Output at 256x256}
    \makebox[\subboxsize]{Output at 480x640}
    \makebox[\subboxsize]{Ground Truth}
        \makebox[\subboxsize]{}
    \makebox[\subboxsize]{}
    \makebox[\subboxsize]{using shad. matte interpolation}
    \makebox[\subboxsize]{}

    \caption{\textbf{Examples of using shadow matte interpolation for shadow removal on high-resolution images.} We show the input shadow images, the results of our model with the shadow parameters and shadow mattes computed using the images of size 256x256. We then interpolate the shadow mattes into the size of the original images (480x640). The third column shows the shadow removal results using these interpolated shadow mattes. The last column shows the adjusted shadow-free images. \textit{(Please magnify the images on a digital device to better view the resolution differences.)}
    }
    \label{fig:highres}
\end{figure}

\subsection{Dataset Augmentation via Shadow Editing}
\label{sec:aug}
Many deep learning work focus on learning from more easily obtainable, weakly-supervised, or synthetic data \cite{Buhmann12weak,LeICCV2017,Liu2014FashionPW,Liu2013WeaklySupervisedDC,appleShrivastavaPTSW16,m_Le-etal-ECCV18,Le_2019_CVPR_Workshops}. In this section, we show that we can modify shadow effects  using our proposed illumination model to generate additional training data. 

Given a shadow matte $\alpha$, a shadow-free image, and  parameters $(w,b)$, we can form a shadow image by:
\begin{equation}
    I^{\textrm{shadow}} = I^{\textrm{shadow-free}}\cdot \alpha + I^{\textrm{darkened}}\cdot (1-\alpha) \\
    \label{eq:aug}
\end{equation}

\noindent where $I^{\textrm{darkened}}$ has undergone the shadow effect associated to the set of shadow parameters $(w,b)$. Each pixel $i$ of $I^{\textrm{darkened}}$ is computed by:
\begin{equation}
I_i^{\textrm{darkened}} = (I_i^{\textrm{shadow-free}}-b) \cdot w^{-1}
\end{equation}

 %Based on this mechanic, we edit the shadow in the training set of the ISTD dataset. We perform a simple procedure.
For each training image, we first compute the shadow parameters and the matte layer via Eqs. \ref{eq:trans} and \ref{eq:alpha}. %We then multiply the computed scaling factor $w$ by a value $k$ to obtain a synthetic scaling factor $w_{\textrm{syn}} = w \times k$. %The shadow image associated to this scaling factor $w_{\textrm{syn}}$ is computed via Eq.\ref{eq:aug}.
Then, we  generate a new synthetic shadow image via Eq. \ref{eq:aug} with a scaling factor $w_{\textrm{syn}} = w \times k$. 
As  seen in Fig. \ref{fig:aug}, a lower $w$ leads to an image with a lighter shadow area while a higher $w$  increases the shadow effects instead. 
Using this method, we augment the ISTD training set by simply choosing $k=\left[0.8,0.9,1.1,1.2\right]$ to generate a new set of 5320 images, which is four times bigger than the original training set.
We augment the original ISTD dataset with this dataset.
 Training our model on this new augmented ISTD dataset improves our results, as the RMSE drops by 6\%, from 7.9 to 7.4, as reported in Tab. \ref{tab:all}. %search for instances were Table was incorrectly abreviated to Tab. and fix them

\def\subboxsize{0.3\subFigSzab}
\begin{figure}[]
 \centering
    \includegraphics[width=0.45\textwidth]{fig/augment.pdf}
     \makebox[\subboxsize]{Syns. Image}
    \makebox[\subboxsize]{Real Image}
    \makebox[\subboxsize]{Syns. Image}
        \makebox[\subboxsize]{ $w_{\textrm{syn}}=w\times 0.8$}
    \makebox[\subboxsize]{ }
    \makebox[\subboxsize]{$w_{\textrm{syn}}=w\times 1.7$}
    \caption{\textbf{Shadow editing via our decomposition model.} We use Eq. \ref{eq:aug} to generate synthetic shadow images. As we change the shadow parameters, the shadow effects change accordingly. %We can obtain a synthetic image with less shadow effect by using a smaller scaling factor $w$ and vice versa. 
    We show two example images from the ISTD training set where in the middle column are the original images and in the first and last column are synthetic.
    }
    \label{fig:aug}
\end{figure}

\begin{table}[]

\centering
\caption{\textbf{Shadow removal results of our networks train on the augmented ISTD dataset.} The metric is RMSE (the lower, the better).  Training our framework on the augumented ISTD dataset drops the RMSE on the shadow area from 7.9 to 7.4. }
\begin{tabular}{lcccc}
\toprule
Methods        &Train. Set            & Shad. & Non-Shad.& All  \\ 
%\midrule
%\multicolumn{4}{c}{Our method trained on the ISTD dataset \cite{Wang_2018_CVPR}}\\
%\midrule
%SP-Net &ISTD & 9.5  &3.2 &4.1\\ 
%SP+M-Net &ISTD  & 7.9  &\textbf{3.1} &3.9\\
%\midrule
%\multicolumn{4}{c}{Our method trained on the aug. ISTD dataset (Ours)}\\
\midrule
SP-Net &Aug. ISTD & 9.0  &3.2 &4.1\\ 
SP+M-Net &Aug. ISTD  & 7.4  &3.1 & 3.8\\
\midrule

%SP+M-Net GT Mask. & 7.4  &2.8 &3.6\\ 
%SP+M-Net + GT Mask  & 7.0  &2.9 &3.5\\\hline
\end{tabular}
\label{tab:all}
\end{table}
